Containment of Shape Expression Schemas for RDF

We study the problem of containment for shape expression schemas (ShEx) for RDF graphs. We identify a subclass of ShEx that has a natural graphical representation in the form of shape graphs and their semantics is captured with a tractable notion of embedding of an RDF graph in a shape graph. When applied to pairs of shape graphs, an embedding is a sufficient condition for containment, and for a practical subclass of deterministic shape graphs, it is also a necessary one, thus yielding a subclass with tractable containment. While for general shape graphs a minimal counter-example i.e., an instance proving non-containment, might be of exponential size, we show that containment is EXP-hard and in coNEXP. Finally, we show that containment for arbitrary ShEx is coNEXP-hard and in coTwoNEXP^NP.

==> hardness.tex <==
\section{Hardness of containment}
\label{sec:hardness}
In this section we investigate what is difficult about testing containment and
we begin by focusing on the classes of \RBEs used in shape expressions. We
present a decision problem parameterized by a class of \RBEs whose complexity
yields a lower bound on complexity of containment of schemas with shape
expression from the same class. We recall that \RBEs have higher computational
requirements than regular expression: testing whether a bag belongs to a
language defined by an \RBE is NP-complete~\cite{} but is in PTIME if we
restrict attention to \RBEZero or single-occurrence \RBEs~\cite{}.

The problem in question is \emph{union-containment} for a class $\C$ of \RBEs
where on the input we have a non-empty sequence of expressions
$E_0,E_1,\ldots,E_n\in\C$ and the question is whether
$L(E_0)\subseteq{}L(E_1\mid\ldots\mid{}E_n)$. We show that the containment for
$\ShEx(\C)$ is at least as hard as union-containment for $\C$.

\begin{lemma}
  If union-containment for $\C$ is hard for a complexity class, then so is
  containment of $\ShEx(\C)$ (under logarithmic reductions).
\end{lemma}
\begin{proof}
  The proof follows the idea behind example in
  Figure~\ref{fig:embedding-does-not-imply-inclusion}. In general, one can
  easily show that $E_0\subseteq{}E_1\cup\ldots\cup{}E_n$ iff the schema with
  the rules $t\rightarrow z\dbl t_0\shuffle [E_0]^{\dbl{}t_0}$ and is contained
  by the schema with the rule
  $t\rightarrow z\dbl t_0 \shuffle [E_1]^{\dbl{}t_0}\shuffle\ldots\shuffle
  [E_n]^{\dbl{}t_0}$, where $[E]^{\dbl{}t_0}$ is obtained by replacing in $E$
  every symbol $a$ by $a\dbl{}t_0$ and $t_0$ has the default definition
  $t_0 \rightarrow \epsilon$. Here $z$ is a fresh symbol not used in any of the
  \RBEs and the component $z\dbl t_0$ ensures that empty bags are handled
  properly.
\end{proof}

\begin{theorem}
  Union-containment for \RBEZero is NP-hard, and consequently, containment for
  \ShExZero is NP-hard. 
\end{theorem}

\begin{theorem}
  Containment for \ShEx is \TWOcoNEXPTIME-hard. 
\end{theorem}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> shape-graphs.tex <==

\section{Shape graphs}
\label{sec:shape-graphs}

\begin{definition}
  \label{def:shape-graphs}
  A \emph{shape} graph is a graph $G$ that additionally comes with
  function $\occur:E_G\rightarrow\I$ that identifies the
  \emph{occurrence} interval of every edge. By $\ShExZero$ we denote
  the class of shape graphs that uses only basic intervals
  in $\M$. \qed
\end{definition}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> trash.tex <==

We define an oriented hypergraph $\G_R$ whose nodes are possible \RBEZero of
width bounded by $n$ and using only atoms of the form $a\dbl{}t^M$, where
$a\in\Sigma$, $t\in N_H\cup H_K$, and $M\in\{\ONE,\MAYBE,\MANY\}$. The nodes of
$\G_R$ are connected using oriented hyperedges, a generalization of simple
oriented edges, where a node is connected simultaneously to one or more nodes,
denoted by $E\rightarrow \{E_1,\ldots, E_k\}$. Intuitively, such a hyperedge
shall capture the fact that a type definition $E$ is covered by
$E_1\cup\ldots\cup E_k$. To define the precise set of the hyperedges of $\G_R$
we begin with an auxiliary relation $\rightarrow_R$ that maps \RBEZero atoms to
sets of \RBEZero's and captures:
\begin{enumerate}
\itemsep0pt
\item the disjunction from $R$, for
  $(t,\{s_1,\ldots,s_m\})\in R$
\begin{align*}
  &a\dbl{}t^\MANY \rightarrow_R \{a\dbl{}s_1^\MANY\shuffle \ldots
    \shuffle a\dbl{}s_m^\MANY\}\\
  &a\dbl{}t^M \rightarrow_R \{a\dbl{}s_1^M,\ldots,a\dbl{}s_m^M\}\qquad
  M\in\{\ONE,\MAYBE\}
\intertext{
\item the disjunction from \RBEZeros
}
&a\dbl{}t^\MAYBE\rightarrow_R \{\epsilon,a\dbl{}t\}\\
&a\dbl{}t^\MANY\rightarrow_R \{\epsilon,a\dbl{}t\shuffle a\dbl{}t^\MANY\}
% \intertext{
% \item the nature of embedding
% }
% &\epsilon\rightarrow_R a\dbl t^\MAYBE\\
% &a\dbl{}t \rightarrow_R a\dbl{}t^\MAYBE\\
% &a\dbl{}t \rightarrow_R a\dbl{}t^\MANY
\end{align*}
\end{enumerate}
Now, the hypergraph $\G_R$ has the hyperedge 
\[
e\shuffle E \rightarrow \{e_1\shuffle E, \ldots, e_m\shuffle E\}
\]
whenever $e\rightarrow_R \{e_1,\ldots,e_m\}$ and the graph $\G_R$
contains the nodes $e\shuffle E, e_1\shuffle E, \ldots, e_m\shuffle E$
for some \RBEZero $E$.

Now, a \emph{tree} in the hypergraph $\G_R$ is a subset of its hyperedges with a
distinguished root node and a set of leaf nodes defined in a recursive fashion:
1) any hyperedge $E\rightarrow X$ of $G$ is a tree with root node $E$ and leaves
$X$; 2) for a tree $S$ with root $E_r$ and leaves $L$, and a hyperedge
$E\rightarrow X$ such that $E\in L$, the set $S\cup\{E\rightarrow X\}$ is a tree
with root $E_r$ and leaves $L\minus\{E\}\cup X$. A tree $S$ is \emph{covered} by
a set of expressions $T$ if for every leaf $E$ of the tree there is $E'\in T$
such that $E\subseteq E'$.
\begin{lemma}
  For any two shape graphs $H$ and $K$, the covering of $H$ by $K$ is
  the maximal relation with $R\subseteq N_H\times \P(N_K)$ with the
  property that for any $(t,T)\in R$, the hypergraph $\G_R$ has a tree
  with root $\delta_H(t)$ and is covered by $\{\delta_K(t')\mid t'\in T\}$.
\end{lemma}

We define an oriented hypergraph $\G_R$ whose nodes are possible \RBEZero of
width bounded by $n$ and using only atoms of the form $a\dbl{}t^M$, where
$a\in\Sigma$, $t\in N_H\cup H_K$, and $M\in\{\ONE,\MAYBE,\MANY\}$. The nodes of
$\G_R$ are connected using oriented hyperedges, a generalization of simple
oriented edges, where a node is connected simultaneously to one or more nodes,
denoted by $E\rightarrow \{E_1,\ldots, E_k\}$. Intuitively, such a hyperedge
shall capture the fact that a type definition $E$ is covered by
$E_1\cup\ldots\cup E_k$. To define the precise set of the hyperedges of $\G_R$
we begin with an auxiliary relation $\rightarrow_R$ that maps \RBEZero atoms to
sets of \RBEZero's and captures:
\begin{enumerate}
\itemsep0pt
\item the disjunction from $R$, for
  $(t,\{s_1,\ldots,s_m\})\in R$
\begin{align*}
  &a\dbl{}t^\MANY \rightarrow_R \{a\dbl{}s_1^\MANY\shuffle \ldots
    \shuffle a\dbl{}s_m^\MANY\}\\
  &a\dbl{}t^M \rightarrow_R \{a\dbl{}s_1^M,\ldots,a\dbl{}s_m^M\}\qquad
  M\in\{\ONE,\MAYBE\}
\intertext{
\item the disjunction from \RBEZeros
}
&a\dbl{}t^\MAYBE\rightarrow_R \{\epsilon,a\dbl{}t\}\\
&a\dbl{}t^\MANY\rightarrow_R \{\epsilon,a\dbl{}t\shuffle a\dbl{}t^\MANY\}
% \intertext{
% \item the nature of embedding
% }
% &\epsilon\rightarrow_R a\dbl t^\MAYBE\\
% &a\dbl{}t \rightarrow_R a\dbl{}t^\MAYBE\\
% &a\dbl{}t \rightarrow_R a\dbl{}t^\MANY
\end{align*}
\end{enumerate}
Now, the hypergraph $\G_R$ has the hyperedge 
\[
e\shuffle E \rightarrow \{e_1\shuffle E, \ldots, e_m\shuffle E\}
\]
whenever $e\rightarrow_R \{e_1,\ldots,e_m\}$ and the graph $\G_R$
contains the nodes $e\shuffle E, e_1\shuffle E, \ldots, e_m\shuffle E$
for some \RBEZero $E$.

Now, a \emph{tree} in the hypergraph $\G_R$ is a subset of its hyperedges with a
distinguished root node and a set of leaf nodes defined in a recursive fashion:
1) any hyperedge $E\rightarrow X$ of $G$ is a tree with root node $E$ and leaves
$X$; 2) for a tree $S$ with root $E_r$ and leaves $L$, and a hyperedge
$E\rightarrow X$ such that $E\in L$, the set $S\cup\{E\rightarrow X\}$ is a tree
with root $E_r$ and leaves $L\minus\{E\}\cup X$. A tree $S$ is \emph{covered} by
a set of expressions $T$ if for every leaf $E$ of the tree there is $E'\in T$
such that $E\subseteq E'$.
\begin{lemma}
  For any two shape graphs $H$ and $K$, the covering of $H$ by $K$ is
  the maximal relation with $R\subseteq N_H\times \P(N_K)$ with the
  property that for any $(t,T)\in R$, the hypergraph $\G_R$ has a tree
  with root $\delta_H(t)$ and is covered by $\{\delta_K(t')\mid t'\in T\}$.
\end{lemma}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

